Stability of the one electron atom Schr\"odinger model with magnetic field in two dimensions

We study the stability of the one electron atom Schr\"odinger model with self-generated magnetic field in two dimensions. The magnetic energy is taken of the general form $K\int_{\mathbb{R}^2} |B|^p$ and we study the stability of the model as a function of the power $p$ and the coupling constant $K$. We show that for $p>3/2$, the model is always stable, and for $p<3/2$, the model is always unstable. In the critical case $p=3/2$, there is a critical stability constant $K_c$, that we characterize in terms of zero modes of the Dirac-Weyl operator. The value of $K_c$ is approximated using analytic and numerical methods.

==> sections/counter-example.tex <==

For $p = 2$, we cannot  control $\norm{\mathbf{A}}_\infty$ by $\norm{B}_2$. Indeed, consider for example 
\begin{equation*}
    B(\mathbf{x}) = \left\{
       \begin{array}{ll}
        \frac{1}{|\x|\log(|\x|)} &  x \in C\\[3mm]
          0 & x \notin C,
          \end{array}
  \right.
\end{equation*}
where $C$ is a sector as in Figure~\ref{fig:my_label}, with $\alpha<\pi$. 
\begin{figure}[ht]
    \centering
    \centering
\begin{tikzpicture}[scale = .5]
    \draw (0,0) -- (5, -5) ;
    \draw  (5, -5) arc (-45: 45: 7.07cm);
    \draw (5, 5) -- (0, 0);
    \draw[<->] (1, 1) arc (45: -45: 1.41cm) node[circle] at (1.7, 0){$\alpha$};
    \draw node[anchor = east] at (0, 0) {$(0, 0)$};
    \draw node at (5, 0){C};
    \draw[thick, <->] (-.5, .5) -- (4.5, 5.5); 
    \draw node[anchor = south east] at (2, 3) {$\frac{1}{2}$};
\end{tikzpicture}
    \caption{The support of the magnetic field $B$}
    \label{fig:my_label}
\end{figure}
The magnetic field $B \in L^2(\mathbb{R}^2)$ but $\left\|\mathbf{A}\right\|_\infty = +\infty$. Indeed,
\begin{equation*}
    \int_{\mathbb{R}^2} |B(\mathbf{x})|^2d\mathbf{x}
   = 2\alpha \log(2),
\end{equation*}
and for $\x$ such that $x_1\geq 0$ and $\av{\x}<1/2$, we have
\begin{align*}
    {A}_2(\x) &= \int_C  \frac{x_1-y_1}{|\mathbf{\x-\y}|^2} B(\mathbf{y})d\mathbf{y}
    \leq -\int_C  \frac{y_1}{|\mathbf{\x-\y}|^2} B(\mathbf{y})d\mathbf{y}\\
&   \leq \int_0^{1/2}     \int_{-\alpha/2}^{\alpha/2}  \frac{r\cos(\theta)}{\av{r-\av{\x}}^2}\frac{1}{r\log(r)}r d\theta dr\\
&= -2\sin(\alpha/2)\int_0^{1/2} \frac{r}{\av{r-\av{\x}}} \frac{1}{\av{r-\av{\x}} \log(r)} dr\\
&\leq -C\int_0^{1/2} \frac{1}{\av{r-\av{\x}} \log(r)} dr\\
    =           -\infty
\end{align*}
So $|\mathbf{A}(0)| = +\infty$

\medskip

Nevertheless, if $B$ is  radial, we exploit the symmetry to extend the inequality to the case $p = 2$.

\begin{theorem}
Let $B \in L^2(\mathbb{R}^2)$ a radially symmetric magnetic field. then, there exists a corresponding vector potential $\mathbf{A}$, such that $div(\mathbf{A}) = 0$ and $curl(\mathbf{A}) = B$. Moreover, 
\begin{equation}
    \left\|\A\right\|_\infty \leq \frac{1}{2\sqrt{\pi}} \left\|B\right\|_2
\end{equation}
\end{theorem}

\begin{proof}
Let $\A$ be defined as in~\eqref{eq:defA}. The symmetries of the problem force the
field $\A$ to have tangential direction with a radial magnitude 
    \begin{equation*}
    \mathbf{A}(\mathbf{x}) = \pm |\mathbf{A}(\mathbf{x})|\mathbf{e}_\theta=\pm |\mathbf{A}(|\mathbf{x}|)|\mathbf{e}_\theta.
\end{equation*}
We integrate $\A$ over the circle of radius $r$ centred at the origin, and apply Stokes theorem to obtain  $$\left| 2\pi r \A(r)\right| = \left|\int_{B(0, r)} B(\mathbf{x}) d\mathbf{x}\right|\leq \sqrt{\pi}r \norm{B}_{2}. $$
This concludes the proof of the theorem. 
\end{proof}

==> sections/diamagnetic-inequality.tex <==

\begin{theorem}
    For a zero mode we have the improved diamagnetic inequality
    \begin{equation}\label{eq:diamagnetic}
    |(\p + \A)\psi|^2 \geq 2|\, \nabla|\psi|\,|^2
\end{equation}
\end{theorem}
\begin{proof}
For no vanishing values of  $\psi$ There is a unitary  $\xi \in \CC^2$ with $|\xi| = 1$ such that 
$$\psi = |\psi|.\xi$$
By the chain rule we have

$$\nabla \psi = \nabla|\psi|.\xi + |\psi|.\nabla\xi$$
Since $\nabla|\psi| \in \RR^2$ So there is a unitary vector $\u \in \RR^2$  $|\u| = 1$ such that $$\nabla|\psi|=|\nabla|\psi||\u$$
We obtain
\begin{equation}\label{eq:dia}
    \nabla \psi = |\nabla|\psi||.\u\otimes\xi + |\psi|.\nabla \xi  
\end{equation}

We have $\xi\cdot\bar{\xi} = 1$, So $\nabla \xi\cdot \bar{\xi} + \nabla\bar\xi\cdot \xi = 0$ which means the vanishing of the real part of 
$$\real{\nabla \xi\cdot \bar{\xi}} = 0$$

Now we take the real value of \textbf{the inner product} of both sides of the equation~\eqref{eq:dia} with the tensor $\mathbf{u}\otimes \bar{\xi}$ 

since $\u$ and $\xi$ are unitary  we obtain,
\begin{equation}\label{eq:norm_gradient}
    \real{\nabla\psi \cdot \u\otimes \bar{\xi}} = |\nabla|\psi|| +  \real{|\psi|\nabla\xi\cdot\u\otimes\bar{\xi}}
\end{equation}

 
But we have 
$$\nabla\xi\cdot\u\otimes \bar{\xi} = u\cdot (\nabla\xi.\bar{\xi})$$

Hence 
$$\real{\nabla\xi\cdot\u\otimes \bar{\xi}} = u\cdot \real{\nabla\xi.\bar{\xi}} = 0$$

The equation~\eqref{eq:norm_gradient} yields
$$|\nabla|\psi|| = \real{\nabla\psi\cdot u\otimes\bar{\xi}}$$


$$\A\otimes\psi\cdot \u\otimes\bar{\xi}  = \langle\A\cdot\u \rangle .\underbrace{\langle \psi \cdot \bar{\xi} \rangle}_{= |\psi|} \in \RR$$

We find that $\real{i\A\otimes\psi\cdot \u\otimes\bar{\xi} } = 0$, So we could add it to the expression  of $|\nabla|\psi||$ without affecting its value, we obtain
$$|\nabla|\psi|| = \real{(\nabla  + i\A)\psi \cdot u\otimes\bar{\xi}}$$


Now let's define the projector $P$ on $\RR^2\otimes\CC^2$ such that 
for  a vector $\mathbf{v}$ and a spinor $\psi$ 
\begin{equation}
    P\parent{\mathbf{v}\otimes \psi } = I - \frac{1}{2} \bsigma\parent{\bsigma\cdot\mathbf{v}}\psi
\end{equation}
For a zero mode $\psi, \A$ we could easily verify that 
$$P((\nabla  + i\A)\psi) = (\nabla  + i\A)\psi$$

We  write the matrix of the this application in the basis $(e_i\otimes \xi_j)$ of $\RR^2\otimes \CC^2$

\begin{equation*}
   \frac{1}{2} \begin{pmatrix}
        1 & 0 & -i & 0\\
        0 & 1 & 0 & i\\
        i & 0 & 1 & 0\\
        0 & -i & 0 & 1
    \end{pmatrix}
\end{equation*}
Which could be easily verify that it is a matrix of an orthogonal projector, and for each $\u\otimes\xi $
$$|P(\u\otimes\xi)| = \frac{1}{\sqrt{2}}|\u||\xi|$$

Now we return to 
\begin{align*}
    |\nabla|\psi|| &= \real{(\nabla  + i\A)\psi \cdot u\otimes\bar{\xi}}\\
    &= \real{(P(\nabla  + i\A)\psi) \cdot u\otimes\bar{\xi}}\\
    &= \real{(\nabla  + i\A)\psi \cdot P (u\otimes\bar{\xi})}\\
    &\leq |(\nabla  + i\A)\psi|\frac{1}{\sqrt{2}}\underbrace{|\u||\xi|}_{= 1}\\
    &\leq \frac{1}{\sqrt{2}}|(\nabla  + i\A)\psi|
\end{align*}



Which is the desired result



\end{proof}



